A Detection and Filtering Framework for Collaborative Localization

Increasingly, autonomous vehicles (AVs) are becoming a reality, such as the Advanced Driver Assistance Systems (ADAS) in vehicles that assist drivers in driving and parking functions with vehicles today. The localization problem for AVs relies primarily on multiple sensors, including cameras, LiDARs, and radars. Manufacturing, installing, calibrating, and maintaining these sensors can be very expensive, thereby increasing the overall cost of AVs. This research explores the means to improve localization on vehicles belonging to the ADAS category in a platooning context, where an ADAS vehicle follows a lead "Smart" AV equipped with a highly accurate sensor suite. We propose and produce results by using a filtering framework to combine pose information derived from vision and odometry to improve the localization of the ADAS vehicle that follows the smart vehicle.

==> subsections/acknowledgement.tex <==
This work was supported by a grant from Ford Motor Company via the Ford-UM Alliance under award N028603. %This work was done as part of ROB590 - Directed Study requirements. The authors thank the University of Michigan - Ann Arbor for the resources and support provided. 

==> subsections/perception.tex <==
% A number of efforts were undertaken to detect the center point of the vehicle. Unfortunately, complications arose with each attempt, ultimately resulting in the abstraction of perception into ground truth within our implementation of the pipeline, shelving perception for future work.
% \paragraph{Single Object Tracking}
%     The first method attempted to obtain the center point of the vehicle via Single Object Tracking, or SOT. This approach involves initializing a 2D bounding box around an object to track, and then running a deep learning network to preserve that bounding box around the object through the image frames or video in which the object is present. In this context, SiameseRPN was used via the MMTracking repository to track the smart vehicle via the ADAS vehicle's front left camera feed.\\
%     In theory, the distance to the smart vehicle can be calculated as follows:
%     \begin{equation}
%     dist_{est} = \frac{W * F}{P}
%     \end{equation}
%     where $W$ represents the known width of the vehicle, $F$ represents the focal length of the camera, and $P$ represents the width of the vehicle in pixels on the camera feed. $F$ can be calculated as follows:
%     \begin{equation}
%         F = \frac{P * dist_{known}}{W}
%     \end{equation}
%     where $dist_{known}$ represents a known distance to the smart vehicle. This value was obtained via the ground truth distance at the first frame of the utilized log.
%     While this appeared to be effective and was relatively simple to implement, the issue of orientation of the smart vehicle with respect to the ADAS vehicle ultimately made this approach infeasible to have an accurate distance estimate to the smart vehicle.\\\\

%     \begin{figure}
%     \includegraphics[width=0.4\columnwidth,scale=1]{Images/car1.JPG}
%     \includegraphics[width=0.5\columnwidth,scale=1]{Images/car2.JPG}
%     \caption{Two frames of the smart vehicle at different angles with respect to the ADAS vehicle}
%     \label{fig:Trajectory of ADAS Vehicle orie_basic}
%     \end{figure}
% As can be seen from the above images, the known width $W$ of the smart vehicle changes when its orientation with respect to the ADAS vehicle changes. Thus, $W$ is not a static parameter and must be estimated with the SOT approach. It was determined due to this that it would be a better approach to estimate the center point of the vehicle in each frame via bounding box, generated by 3D object detection methods, and do so in a manner that can return bounding box coordinates in 3D space, and not just pixel coordinates. 

% \paragraph{Frame-by-Frame Object Detection w/ Depth Estimation}
%     The second attempt on estimating the distance to the smart vehicle to assist localization efforts was estimating a point cloud and applying it to an object detection network. The particular implementation chosen was the Pseudo-LiDAR method, which was joined with aggregate view object detection (AVOD) for 3D detection and visualization. This would in theory locate the center point of the smart vehicle (regardless of orientation with respect to the ADAS vehicle) and provide coordinates for it in 3D space, allowing for a simple calculation to obtain the distance to that point. Although the Pseudo-LiDAR files were generated successfully from image frame data, the paired detection method (AVOD) did not work due to dependency issues. Our setup ran on Ubuntu 20.04 with GPUs designed for the newest CUDA versions, whereas AVOD was created in 2018 and runs on legacy versions of CUDA that required an older version of Ubuntu, and even more problematic, older GPUs. As this required a complete switch of hardware, this approach was also deemed infeasible. Due to time constraints, a proper method of distance estimation was not found in time, and ground truth values were elected to be used as a "simulation" of perception. \
    % Ground truth pose of the ADAS vehicle - $P_W^C$ \\
    % Ground truth pose of the SMART vehicle - $P_W^S$ \\
    % ADAS vehicle in the frame of the SMART vehicle - $P_S^C$\\
    % Translation along x and y - T \\
    % Rotations as Quaternions - R \\

    
    
